The ROMES method for statistical modeling of reduced-order-model error

This work presents a technique for statistically modeling errors introduced by reduced-order models. The method employs Gaussian-process regression to construct a mapping from a small number of computationally inexpensive `error indicators' to a distribution over the true error. The variance of this distribution can be interpreted as the (epistemic) uncertainty introduced by the reduced-order model. To model normed errors, the method employs existing rigorous error bounds and residual norms as indicators; numerical experiments show that the method leads to a near-optimal expected effectivity in contrast to typical error bounds. To model errors in general outputs, the method uses dual-weighted residuals---which are amenable to uncertainty control---as indicators. Experiments illustrate that correcting the reduced-order-model output with this surrogate can improve prediction accuracy by an order of magnitude; this contrasts with existing `multifidelity correction' approaches, which often fail for reduced-order models and suffer from the curse of dimensionality. The proposed error surrogates also lead to a notion of `probabilistic rigor', i.e., the surrogate bounds the error with specified probability.

==> definitions/commands_diff.tex <==
\ifthenelse{\equal{\atype}{siam}}{
\bibliographystyle{siam}
}{%
\usepackage{amsthm}
\bibliographystyle{siam}
\newcommand{\diag}{\mathrm{diag}}
}

\newtheorem{remark}{Remark}[section]

\ifthenelse{\equal{\atype}{siam}}
{
\newcommand{\itemname}{romannum}
}
{
\newcommand{\mref}[1]{(\ref{#1})}
\newcommand{\itemname}{itemize}
}


%
\definecolor{Blue}{rgb}{0,0,1}
\definecolor{Red}{rgb}{1,0,0}
\definecolor{Orange}{rgb}{1,0,1}
%
\newcommand{\KTC}[1]{{\textcolor{Blue}{KTC: #1}}}
\newcommand{\MD}[1]{{\textcolor{Orange}{MD: #1}}}
\newcommand{\highlight}[1]{{\textcolor{Red}{#1}}}
\newcommand{\cb}[1]{\left\{#1\right\}}
\newcommand{\rb}[1]{\left(#1\right)}
\newcommand{\eb}[1]{\left[#1\right]}
\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\detI}{\ensuremath{\text{h}}}
\newcommand{\redI}{\ensuremath{\text{red}}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\enorm}[1]{\vertiii{#1}}
\newcommand{\xnorm}[1]{\norm{#1}_{X_{\detI}}}
\newcommand{\K}{\mathbf{K}}

\newcommand{\bt}{\mathbf{t}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\abs}[1]{\left|#1\right|}

\def \pat#1{{\bf #1}}
\def \cal{\mathcal}
\newcommand{\balpha}{{\bm \alpha}}
\newcommand{\bnu}{{\bm \nu}}
\newcommand{\barnu}{{\bar \nu}}
\newcommand{\bbarnu}{{\bar {\bm\nu}}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bmu}{{\bm \mu}}
\newcommand{\inputs}{{\bmu}}
\newcommand{\params}{{\inputs}}
\newcommand{\paramTrain}[1]{{\inputs}_{#1}}
\newcommand{\paramsOnline}{{\inputs}^\star}
\newcommand{\nTrain}{N}
\newcommand{\bmutrain}{\tilde{\bm \mu}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bbarSigma}{\bar{\mathbf{\Sigma}}}
%
\newcommand{\bbaralpha}{\boldsymbol{\bar \alpha}}
\newcommand{\field}[1]{ \mathbb{#1} }
\usepackage{mathtools}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\leftbasis}{\ensuremath{\bm{W}}}
\newcommand{\rightbasis}{\ensuremath{\bm{V}}} 
\newcommand{\rightbasisfine}{} 
\newcommand{\redstatefine}{\state} 
\newcommand{\rightbasiscoarse}{\rightbasis} 
\newcommand{\rightbasisdualcoarse}{\bm{Y}} 
\newcommand{\rightbasiscoarseT}{\rightbasis^T} 
\newcommand{\rightbasisdualcoarseT}{\rightbasisdualcoarse^T} 
\newcommand{\redstatecoarse}{\redstatecoords} 
\newcommand{\nat}{\mathbb{N}} 
\newcommand{\errorIndicatorFinei}{\delta} 
%
\newcommand{\rightbasisfineT}{} 
\newcommand{\range}[1]{\ensuremath{\mathrm{range}\left(#1\right)}}
\newcommand{\RR}{ \field{R} }
\newcommand{\NN}{ \field{N} }
\newcommand{\CC}{ \field{C} }
%
\newcommand{\cF}{ {\cal F} }
\newcommand{\cX}{ {\cal X} }
\newcommand{\cP}{ {\cal P} }
\newcommand{\cM}{ {\cal M} }
\newcommand{\cR}{ {\cal R} }
\newcommand{\cI}{ {\cal I} }
\newcommand{\cT}{ {\cal T} }
\newcommand{\cH}{ {\cal H} }
\newcommand{\cN}{ {\cal N} }
\newcommand{\cG}{ {\cal G} }
\newcommand{\cW}{ {\cal W} }
\newcommand{\cL}{ {\cal L} }
\newcommand{\cD}{ {\cal D} }
\newcommand{\cS}{ {\cal S} }
\newcommand{\cO}{ {\cal O} }
\newcommand{\caG}{ \cal G }
\newcommand{\myspan}{ \mathrm{span} }
\newcommand{\Id}{ \mathrm{Id} }
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\card}[1]{\mathrm{card}\left(#1\right)}
%
\newcommand{\sgn}{ \mathrm{sgn} }
%
\newcommand{\scalprod}[2]{ \left< #1 , #2 \right> }
\newcommand{\twovec}[2]{\left(\begin{array}{c} #1 \\ #2
    \end{array}\right)}
\newcommand{\bn}{\bf n}

%
%
%
%
%
%


\newcommand{\erf}{\mathrm{erf}}
\newcommand{\rigorbound}{\quantity_\mathrm{LB}}
\newcommand{\crigor}{c}
\DIFaddbegin \newcommand{\cvalidation}{c_\text{validation}}
\DIFaddend \newcommand{\mode}[1]{\mathrm{mode}\rb{#1}}
\newcommand{\median}[1]{\mathrm{median}\rb{#1}}
\newcommand{\contstate}{u}
\newcommand{\contstatedummy}{w}
\newcommand{\contfestate}{\contstate_{\detI}}
\DIFaddbegin \newcommand{\contfedual}{y_{\detI}}
\newcommand{\contfetest}{v_{\detI}}
\DIFaddend \newcommand{\contredstate}{\contstate_{\redI}}
\newcommand{\state}{{\bm{u}}}
\newcommand{\stateH}{\state_{\detI}}
\newcommand{\redstate}{\state_{\redI}}
\newcommand{\dualstate}{{\bm{y}}}
\newcommand{\reddualstate}[1]{\dualstate_{\redI, #1}}
\newcommand{\redstatecoords}{\hat \state}
\newcommand{\statecont}{u}
\newcommand{\out}{s}
\newcommand{\outputs}{\out}
\newcommand{\outputfun}{g}
\DIFaddbegin \newcommand{\outputfunCont}{\bar g}
\newcommand{\outCont}{\bar \out}
\DIFaddend \newcommand{\residual}{\ensuremath{\bm{r}}}
\newcommand{\modresidual}{\residual}
\newcommand{\coarsetofine}{\rightbasis}
\newcommand{\adjoint}{\bm{y}}
\newcommand{\redadjointfine}{\adjoint}
\newcommand{\redadjointcoarsetofine}{\adjoint_{\redI}}
\newcommand{\redadjointcoarsetofineII}{\adjoint_{\redI, i}}
\newcommand{\redadjointcoarsetofinearg}[1]{\adjoint_{\redI, #1}}
\newcommand{\redadjointcoarsetofinei}{\adjoint_i^H}
\newcommand{\redadjointcoarsetofineT}{\rightbasis^{HT}} 
\newcommand{\redadjointcoarse}{\hat\adjoint}
\newcommand{\redadjointfineT}{\adjoint^T}
\newcommand{\nrbfine}{\ndof}
\newcommand{\timestepit}{k}
\newcommand{\residualnorm}{\ensuremath{{r}}}
\newcommand{\residualhyper}{\ensuremath{\tilde\residual}}
\newcommand{\outmeas}{\bar s}
\newcommand{\redout}{\out_{\redI}}
\newcommand{\redoutI}{\out_{i, \redI}}
\newcommand{\outsurr}{\out_{\mathrm{surr}}}
\newcommand{\error}{\delta}
\newcommand{\quantity}{\ensuremath{m}}
\newcommand{\quantitysurr}{\ensuremath{\tilde{\quantity}}}
\newcommand{\statebias}{\delta_{\state}}
\newcommand{\stateerrorvecNo}{{\bm{\delta}_{\state}}}
\newcommand{\stateerrorvec}[1]{\stateerrorvecNo#1}
\newcommand{\stateerror}[1]{\norm{\stateerrorvec{#1}}}
\newcommand{\xstateerror}[1]{\xnorm{\stateerrorvec{#1}}}
%
%
\newcommand{\enstateerror}[1]{\enorm{\stateerrorvec{#1}}}
\newcommand{\outbias}{\delta_{\out}}
\newcommand{\outbiasone}{\delta_{\out_1}}
\newcommand{\outbiastwo}{\delta_{\out_2}}
\newcommand{\outbiasi}{\delta_{\out_i}}
\newcommand{\outbiasMF}{\delta_{\out, \text{MF}}}
\newcommand{\outerror}[1]{\abs{\delta_{\out}{#1}}}
\newcommand{\bound}{\Delta}
\DIFaddbegin \newcommand{\lowerbound}{\Delta^\text{LB}}
\DIFaddend \newcommand{\statebound}{\bound_{\state}}
\DIFaddbegin \newcommand{\statelowerbound}{\lowerbound_{\state}}
\DIFaddend \usepackage{bbm}
\newcommand{\indicator}[2]{{\mathbbm{1}}_{#2}\left(#1\right)}
\newcommand{\cint}{C}
\newcommand{\confidenceInterval}[2]{\cint_{#1}\left(#2\right)}
\DIFaddbegin \newcommand{\confidenceIntervalOne}[1]{\cint_{#1}}
\DIFaddend \newcommand{\indicators}{\bm{\rho}}
\newcommand{\stateindicator}{\bm{\rho}}
\newcommand{\outbound}{\bound_{\out}}
\DIFaddbegin \newcommand{\outlowerbound}{\lowerbound_{\out}}
\DIFaddend \newcommand{\outcorrected}{\out_{\text{corr}}}
\newcommand{\mapdomain}{\cal D}
%
\newcommand{\maprange}{\RR{}}
\newcommand{\inp}{f}
\newcommand{\nindicator}{q}
\newcommand{\Para}{\cP}
\newcommand{\paramDomain}{\Para}
\newcommand{\Paratrain}{\ensuremath{\Para_{\mathrm{train}}}}
\DIFaddbegin \newcommand{\Paragreedy}{\ensuremath{\Para_{\mathrm{greedy}}}}
\newcommand{\romesTraining}{\ensuremath{N}}
\DIFaddend \newcommand{\Pararomes}{\ensuremath{\bar\Para}}
\newcommand{\Paratrainromes}{\ensuremath{\Para_{\mathrm{learn}}}}
\newcommand{\Paravalidate}{\ensuremath{\Para_{\mathrm{validation}}}}
\newcommand{\nparams}{{\ensuremath{n_\params}}}
\DIFaddbegin \newcommand{\nxvars}{\ensuremath{n_{\bm{x}}}}
\DIFaddend \newcommand{\ndof}{\ensuremath{n}}
\newcommand{\Figure}[1]{Figure #1}
\newcommand{\Figures}[1]{Figures #1}
\newcommand{\Section}[1]{Section #1}
\newcommand{\Sections}[1]{Sections #1}
\newcommand{\methodname}{ROMES}%
\newcommand{\rbmatlab}{RBMatlab}
\newcommand{\methodexplanation}{ROM Error Surrogates}%
\newcommand{\stochastic}[1]{\widetilde{#1}}
%
\newcommand{\machine}{\quantitysurr}
\newcommand{\machiney}{\tilde y}
\DIFaddbegin \newcommand{\ciVar}{{\omega}}
\newcommand{\cobs}[1]{{\ciVar_\text{validation}\left(#1\right)}}
\newcommand{\errorSurrUni}{\stochastic{\error_\text{uni}}}
\DIFaddend%
%
\newcommand{\functionErrorNo}{d}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\functionError}[1]{\functionErrorNo(#1)}
\newcommand{\errorsurr}{\tilde \functionErrorNo}
\newcommand{\rbphi}{\psi}
\newcommand{\bphi}{\bm \phi}
\newcommand{\bPhi}{\bm \Phi}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\rvmvar}{k}
\newcommand{\rvmnum}{K}
\newcommand{\Mtrain}{\cM_{\text{train}}}
\DIFaddbegin \newcommand{\Mgreedy}{\cM_{\text{greedy}}}
\DIFaddend \newcommand{\identityFunction}[1]{\mathrm{id}_{#1}}

\newcommand{\nrb}{p}
\newcommand{\nrbdual}{p_y}
\newcommand{\expected}[1]{\ensuremath{\mathrm{E}\eb{#1}}}
\newcommand{\prob}[1]{\ensuremath{\mathrm{P}[#1]}}
\newcommand{\effectivity}{\ensuremath{\eta}}
\newcommand{\effectivityLow}{\ensuremath{\eta_1}}
\newcommand{\effectivityHigh}{\ensuremath{\eta_2}}
\DIFaddbegin \newcommand{\febasisvec}{\ensuremath{\varphi}}
\newcommand{\dirac}{\ensuremath{\delta_\text{Dirac}}}
\newcommand{\coefficientFunction}{\ensuremath{b}}
\DIFaddend%
%
%


==> definitions/tikz.tex <==
\usepackage{tikz}
\usepackage{pgfplots,pgfplotstable}
\usetikzlibrary{calc, positioning, shapes.multipart}

\pgfplotsset{compat=1.8}
\usepgfplotslibrary{external}
\tikzexternalize
\tikzset{external/mode=list and make}
\ifthenelse{\equal{\atype}{siam}}{
\tikzsetexternalprefix{siam_extfigures/}}
{
\tikzsetexternalprefix{extfigures/}}



